Finiteness properties of arithmetic groups over function fields

We determine when an arithmetic subgroup of a reductive group defined over a global function field is of type FP_\infty by comparing its large-scale geometry to the large-scale geometry of lattices in real semisimple Lie groups.

==> figure_1.tex <==
\ProvidesFile{figure_1.tex}
\begingroup
  \setlength{\unitlength}{1cm}
  \setlength{\fboxsep}{0pt}
  \setlength{\fboxrule}{0pt}
  \fbox{%
  \begin{picture}(4,4.1)(-0.5,-0.7)
  %(3.3,3.85)(-0.15,-0.6)
    \put(-0.65,-0.1){\includegraphics{figures.1.ps}{}{}}
    \put(-0.3,0.9){$i$}
    \put(-0.1,-0.5){$0$}
    \put(0.9,-0.5){$1$}
    \put(1.9,-0.5){$2$}
    \put(2.9,-0.5){$3$}
    \put(-0.2,2.8){$\infty$}
  \end{picture}%
  }
\endgroup
\endinput


==> figure_2.tex <==
\ProvidesFile{figure_2.tex}
\begingroup
  \setlength{\unitlength}{1cm}
  \setlength{\fboxsep}{0pt}
  \setlength{\fboxrule}{0pt}
  \fbox{%
  \begin{picture}(3.3,3.9)(-0.15,-0.6)
    \put(-0.05,-0.1){\includegraphics{figures.2}{}{}}
    \put(-0.3,0.45){$x$}
    \put(-0.1,-0.5){$0$}
    \put(.9,-0.5){$t$}
    \put(1.9,-0.5){$t^2$}
    \put(2.9,-0.5){$t^3$}
%\put(2,-0.4){\clap{$t[][\Two]$}}
 %   \put(3,-0.4){\clap{$t[][\Three]$}}
    \put(-.2,2.8){$\infty$}
  \end{picture}%
  }
\endgroup
\endinput

